Reasoning Core: Designing Broad Procedural Data for Completion-Supervised Reasoning Training

Procedural generators produce useful verifiable reasoning problems at scale, but have received less attention as data for completion-supervised fine-tuning. We introduce Reasoning Core, a collection of 50 generators spanning mathematics, logic, planning, state tracking, formal languages, structured data, games, causality, and code, with semantic scorers, difficulty controls, and task evaluators. Under a matched completion-supervised protocol, we compare Reasoning Core with Procedural Warmup, Reasoning Gym, and SynLogic across four base-model settings and multiple training durations. In the primary 3B comparison, Reasoning Core achieves the highest mean scores on DROP, LogiQA, and ARC-Challenge, exceeding both the baseline without procedural data and all three alternative procedural collections. Task-level analyses show that semantic validity alone does not ensure training utility, highlighting compact targets and calibrated difficulty as important design factors. We ran audits combining model-assisted review, human adjudication, and regression testing. Applied throughout Reasoning Core development and to the other collections, they reveal subtle mismatches among generation, rendering, targets, and scoring, a reminder that procedural generation alone does not guarantee correctness. The library, generated datasets, and audit material are publicly available.

==> generated/claims.tex <==
\makeatletter\def\clm#1{\csname clm@#1\endcsname}
\@namedef{clm@free_gen_accuracy_table.drop_rc_1.7B}{-2.2}
\@namedef{clm@free_gen_accuracy_table.drop_rc_OLMo-1B}{+1.7}
\@namedef{clm@free_gen_accuracy_table.drop_rc_SmolLM3-3B}{+3.0}
\@namedef{clm@free_gen_accuracy_table.drop_rgym_1.7B}{-0.2}
\@namedef{clm@free_gen_accuracy_table.drop_rgym_OLMo-1B}{-2.1}
\@namedef{clm@free_gen_accuracy_table.drop_rgym_SmolLM3-3B}{+3.0}
\@namedef{clm@free_gen_accuracy_table.gsm8k_rc_1.7B}{+2.7}
\@namedef{clm@free_gen_accuracy_table.gsm8k_rc_OLMo-1B}{-1.8}
\@namedef{clm@free_gen_accuracy_table.gsm8k_rc_SmolLM3-3B}{+1.6}
\@namedef{clm@free_gen_accuracy_table.gsm8k_rgym_1.7B}{+0.5}
\@namedef{clm@free_gen_accuracy_table.gsm8k_rgym_OLMo-1B}{-0.6}
\@namedef{clm@free_gen_accuracy_table.gsm8k_rgym_SmolLM3-3B}{+1.6}
\@namedef{clm@free_gen_accuracy_table.lead_drop_1.7B}{-2.0}
\@namedef{clm@free_gen_accuracy_table.lead_drop_OLMo-1B}{+3.8}
\@namedef{clm@free_gen_accuracy_table.lead_drop_SmolLM3-3B}{-0.0}
\@namedef{clm@free_gen_accuracy_table.lead_gsm8k_1.7B}{+2.2}
\@namedef{clm@free_gen_accuracy_table.lead_gsm8k_OLMo-1B}{-1.2}
\@namedef{clm@free_gen_accuracy_table.lead_gsm8k_SmolLM3-3B}{+0.1}
\@namedef{clm@heldout_bbh_transfer_table.lead_1.7B}{-1.37}
\@namedef{clm@heldout_bbh_transfer_table.lead_135M}{+0.27}
\@namedef{clm@heldout_bbh_transfer_table.lead_360M}{-0.56}
\@namedef{clm@heldout_bbh_transfer_table.lead_OLMo-1B}{-1.26}
\@namedef{clm@heldout_bbh_transfer_table.lead_SmolLM3-3B}{-15.57}
\@namedef{clm@main_transfer_table.lead_OLMo-1B}{+3.18*}
\@namedef{clm@main_transfer_table.pw_OLMo-1B}{+1.72*}
\@namedef{clm@main_transfer_table.rc_OLMo-1B}{+15.05*}
\@namedef{clm@main_transfer_table.rgym_OLMo-1B}{+11.88*}
\@namedef{clm@main_transfer_table.synlogic_OLMo-1B}{+4.16*}
\@namedef{clm@saturation_reward_table.rc_1.7B}{0.043}
\@namedef{clm@saturation_reward_table.rc_135M}{0.020}
\@namedef{clm@saturation_reward_table.rc_360M}{0.097}
\@namedef{clm@saturation_reward_table.rc_OLMo-1B}{0.269}
\@namedef{clm@saturation_reward_table.rc_SmolLM3-3B}{0.345}
\@namedef{clm@saturation_reward_table.rgym_1.7B}{0.001}
\@namedef{clm@saturation_reward_table.rgym_135M}{0.017}
\@namedef{clm@saturation_reward_table.rgym_360M}{0.052}
\@namedef{clm@saturation_reward_table.rgym_OLMo-1B}{0.130}
\@namedef{clm@saturation_reward_table.rgym_SmolLM3-3B}{0.217}
\@namedef{clm@saturation_reward_table.synlogic_1.7B}{0.000}
\@namedef{clm@saturation_reward_table.synlogic_135M}{0.017}
\@namedef{clm@saturation_reward_table.synlogic_360M}{0.007}
\@namedef{clm@saturation_reward_table.synlogic_OLMo-1B}{0.034}
\@namedef{clm@saturation_reward_table.synlogic_SmolLM3-3B}{0.034}
\@namedef{clm@scale_crossover_ladder.1.7B_T300}{-1.02}
\@namedef{clm@scale_crossover_ladder.135M_T1200}{+0.35*}
\@namedef{clm@scale_crossover_ladder.135M_T2400}{+0.95*}
\@namedef{clm@scale_crossover_ladder.135M_T300}{+1.18}
\@namedef{clm@scale_crossover_ladder.135M_T600}{-1.11}
\@namedef{clm@scale_crossover_ladder.360M_T1200}{-0.73*}
\@namedef{clm@scale_crossover_ladder.360M_T2400}{-0.90*}
\@namedef{clm@scale_crossover_ladder.360M_T300}{+0.40}
\@namedef{clm@scale_crossover_ladder.360M_T600}{-2.76}
\@namedef{clm@scale_crossover_ladder.OLMo-1B_T1200}{+3.18*}
\@namedef{clm@scale_crossover_ladder.OLMo-1B_T300}{+3.34}
\@namedef{clm@scale_crossover_ladder.OLMo-1B_T600}{+1.67}
\@namedef{clm@scale_crossover_ladder.SmolLM3-3B_T1200}{-10.87}
\@namedef{clm@scale_crossover_ladder.SmolLM3-3B_T2400}{-2.52}
\@namedef{clm@scale_crossover_ladder.SmolLM3-3B_T300}{-12.14}
\@namedef{clm@scale_crossover_ladder.SmolLM3-3B_T600}{-11.44}
\makeatother

